Automatic Objects Removal for Scene Completion

With the explosive growth of web-based cameras and mobile devices, billions of photographs are uploaded to the internet. We can trivially collect a huge number of photo streams for various goals, such as 3D scene reconstruction and other big data applications. However, this is not an easy task due to the fact the retrieved photos are neither aligned nor calibrated. Furthermore, with the occlusion of unexpected foreground objects like people, vehicles, it is even more challenging to find feature correspondences and reconstruct realistic scenes. In this paper, we propose a structure based image completion algorithm for object removal that produces visually plausible content with consistent structure and scene texture. We use an edge matching technique to infer the potential structure of the unknown region. Driven by the estimated structure, texture synthesis is performed automatically along the estimated curves. We evaluate the proposed method on different types of images: from highly structured indoor environment to the natural scenes. Our experimental results demonstrate satisfactory performance that can be potentially used for subsequent big data processing: 3D scene reconstruction and location recognition.

==> def.tex <==
\section{Models and Concepts}
\label{sec:def}
%\vspace{-0.1in}

In this section, we introduce our general framework for image completion. First let us define a set of denotations for the rest of paper. As mentioned earlier, the target region for filling is denoted as $\mathbf{\Omega}$; the source part $\mathbf{\phi} (= \mathbf{I} - \mathbf{\Omega})$ is the area whose pixels are known. The boundary contours are denoted as $\mathbf{\partial\Omega}$. A pixel's value is represented by $p = \mathbf{I(x, y)}$, where x and y are the coordinates on image. The surrounding neighborhood centered at $(x, y)$ is written as a patch $\Psi_p$, whose coordinates are within $[x\pm \Delta{x}, y\pm \Delta{y}]$, as shown in Figure \ref{fig:symbols}. In our system model, three important phases are involved:

%\begin{figure}[htb]
%\centerline{\epsfig{figure=pic/Symbols.eps, width=5.5cm}}
%\caption{Symbols Definition}\label{fig:symbols}
%\end{figure}

{\bf Structure Estimation:} In this stage, the input is the original image with $\mathbf{\Omega}$ marked by the user. Image analysis is executed on the known pixels $\mathbf{\phi}$. The aim of this step is to estimate all the possible edges in the unknown area $\mathbf{\Omega}$. Here our strategy is applying \emph{gPb Contour Detector}\cite{Pablo_11} on the images to extract the distribution of edges on the image:

\begin{equation}
I_{edge} = \sqrt{[\frac{\partial}{\partial x}(I \ast G_x)]^2 + [\frac{\partial}{\partial y}(I \ast G_y)]^2}
\end{equation}

Where, $G_x$ and $G_y$ are the first derivative of Gaussian function with respect to $x$ and $y$ directions ($G_x = \frac{-x\cdot G(x, y)}{\sigma^2}$). After computing $I_{edge}$, the main edges on the image can be extracted by threshold suppression.

Now all the edges that intersects with the target region $\mathbf{\partial\Omega}$ can be found. Inspired from \cite{Anal_02}, the edges in $\Omega$ can be estimated by linking matching pairs of edges along the contour. However, there are some potential problems in this scheme. There could be a lot of edges on  $\mathbf{\partial\Omega}$, especially when the size of the missing region is big. The priorities of the edge pairs need be considered in terms of drawing the connecting lines in $\Omega$. Furthermore, what should the chains look like when it connects the edges? Will it be a straight line or a certain curve? The solutions for these problems are described in details in next section.

{\bf Structure Propagation:} After the edges are approximated from last stage, they are propagated across the region before structure propagation. These estimated edges act as the framework in building the whole region. We adopt the idea introduced in \cite{sun_05}, where \emph{Belief Propagation} \cite{Pearl_88} is used to synthesize the estimated structure and respective texture in $\Omega$. However, we have made a few improvements based on our \emph{adaptive patch scheme} During the propagation, exemplar-based technique is employed: similar texture patches from $\mathbf{\phi}$ are copied and pasted along the edges in $\Omega$.

{\bf Final Propagation:} The remaining blank area in $\Omega$ are filled after the structure are drawn. As mentioned in many previous works, the order of rendering pixels is critical in synthesizing the final image. A priority-based patching filling scheme is taken to optimize the natural coherence while preserving variations of shapes.





==> mot.tex <==
\section{Motivational Examples}
\label{sec:mot}
%\vspace{-0.1in}

The process of our framework is like this: for a given image $\mathbf{I}$, the users specify the objects that need to be removed by drawing a closed contour around them. These enclosure is usually denoted as $\mathbf{\Omega}$, which is considered as unknown region on $\mathbf{I}$. In Figure \ref{fig:demo}, the car is selected as the object for removal. In the resulting image, the occluded region is automatically filled  with minimized visual artifact.



Our algorithm is derived from the following observations:spacial coherence among neighboring pixels imposes strong constraints on rendering the unknown region. The definition have been formalized mathematically in  \cite{Criminisi_04}\cite{Efros_01}\cite{Freeman_00}\cite{Efros_99}\cite{Bonet_97}\cite{c_01}\cite{Wey_00}. Exemplar-based approach is well-proved approach for this purpose. However, a naive copy-and-paste of image patches may lead to noticeable artifacts. Thus structure preservation is a key factor in solving this problem. There exists several techniques \cite{sun_05} for structures maintenance. For different images, the above two factors may play different roles in rendering the missing region. According to many previous works \cite{Criminisi_04}, the order of rendering pixels is critical the quality of resulting image.

In our proposed algorithm, we give a formal approach on determining the priorities of the above two factors and also develop an automatic in-painting algorithm.

%more than one choice each time.
%We will filter out unnecessary prefetch.
%According the probability
%in the pattern,  keep useful prefetch.
%For example,
%if $A$ to $B$ is 0.6, a to a is 0.2 and a to c is 0.2. Then
%we can fetch a, b, and c three data at same time. Then
%it nearly 100 percent confidence that there is no cache
%miss.

%It is impossible to find association rule in real-time.
%We must do it at compile time (the regular pattern).
%Then using supervising method to guide the decision.
%We need a large mounts of data. If we use unsupervise
%method we need using cluster method, such as out-liner methods.



%Prefetch engine ( a new thread or a new hardware? Run ahead thread):
%built up table $\to$ data cleaning $\to$

%$\to$ association rule $\to$ regular pattern (loop has regular pattern)
%$\to$ strategies $\to$ benchmarks, how to set up experiments.
%Using CMP (Chip Multiprocessor) to processing data simultaneously.

%A new way is discountinuty prefetch. Which does not have a regular
%pattern.



%Build up a history table is a good way. We count statistically,
%how many time cache miss should go to a, b or c. We always fetch
%the three one with highest should-go rate.














































